Training Data Generating Networks: Shape Reconstruction via Bi-level Optimization

We propose a novel 3d shape representation for 3d shape reconstruction from a single image. Rather than predicting a shape directly, we train a network to generate a training set which will be fed into another learning algorithm to define the shape. The nested optimization problem can be modeled by bi-level optimization. Specifically, the algorithms for bi-level optimization are also being used in meta learning approaches for few-shot learning. Our framework establishes a link between 3D shape analysis and few-shot learning. We combine training data generating networks with bi-level optimization algorithms to obtain a complete framework for which all components can be jointly trained. We improve upon recent work on standard benchmarks for 3d shape reconstruction.

==> images/main.tex <==
\begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=1\linewidth,grid=false]{images/main.png}
\put(0,78){\rotatebox{90}{\tiny{\textbf{Input Images}}}}
\put(0,53){\rotatebox{90}{\tiny{\textbf{Ground Truth}}}}
\put(0,33){\rotatebox{90}{\tiny{\textbf{OccNet}}}}
\put(0,7){\rotatebox{90}{\tiny{\textbf{Proposed}}}}
\end{overpic}

